Transferable Unlearnable Examples

With more people publishing their personal data online, unauthorized data usage has become a serious concern. The unlearnable strategies have been introduced to prevent third parties from training on the data without permission. They add perturbations to the users' data before publishing, which aims to make the models trained on the perturbed published dataset invalidated. These perturbations have been generated for a specific training setting and a target dataset. However, their unlearnable effects significantly decrease when used in other training settings and datasets. To tackle this issue, we propose a novel unlearnable strategy based on Classwise Separability Discriminant (CSD), which aims to better transfer the unlearnable effects to other training settings and datasets by enhancing the linear separability. Extensive experiments demonstrate the transferability of the proposed unlearnable examples across training settings and datasets.

==> sections/backup_intro.tex <==
\section{Introduction}
\label{sec:intro}

% \subsection{Findings}

% \begin{itemize}
%     \item The unlearnable examples can be used to protect data from unauthorized using, but it can only work in one single situation where the poison is generated. 
%     \item The poisoned data generated in a supervised way cannot work when others train with it in an unsupervised way and vice versa. 
%     \item Our main result is that our method can extend unlearnable examples on a labeled dataset to both the supervised setting and the self-supervised setting. 
%     \item We generalize this idea to the unlabeled datasets. When label information is not available, we can use $k$-means to generate the pseudo labels and generate the perturbation with our method by the pseudo labels. We can decrease the performance by 10\% to 20\% if others get our data, annotate it and train on it. We can also get better poisoned performance of unlearnable error-minimizing noise on unsupervised contrastive learning than baseline.
%     \item We have noticed the trade-off between supervised and self-supervised poisoning is not just competing with each other. When we put more weight on one of the poisoning components, the other light component will have positive influence on the weight one instead of decreasing the performance. %(It is possible that transferbility from resnet-18 to VGG11 is also better than supervised unlearnable baseline. I am doing experiments to verify.)
% \end{itemize}

1. wh unlearning is important? 

2. supervised and unsuperivsed unlearning?? 

generation/learning,   supervised,  unsupervised

superivsed         1 x                  x
unsupervised         x                  x 1

why this is a problem

results.. superivsed ---> unsupervised? unsupervised --> superivsed ??  what are the consquences??? importnat to make both supevised and unsuperivsed unlearnbale? 


3. unlearn both, think about challenges and how we solve these challenges

With the emerging of the Internet, more and more data are available online such as pictures posted on social media, and user behaviors on E-commerce websites. Some are public from service providers, while others are personal from individuals. On the one hand, using such data collected from the online resources such as ImageNet, Freebase, and Ms-celeb-1m\cite{deng2009imagenet, bollacker2008freebase, guo2016ms}, deep learning that relies on large-scale training data achieves very promising performance in many real-world applications. On the other hand, private information can be also learned by the deep models without permission in this process~\cite{yeom2018privacy}. Data owners are facing many privacy issues including membership inference,
model inversion, hyperparameter inference, parameter inference, and property inference attacks ~\cite{mireshghallah2020privacy}. When data is not public, it can be protected by key or encryption. But it becomes more challenge to protect the data from unauthorized usage when it is released publicly like the pictures posted on the social platform, because we can not stop attackers from the access to data. Recently, researchers  to make unauthorized deep models only learn useless information by poisoning attack. For example, Huang et al.~\cite{huang2020unlearnable} and Flow et al.~\cite{fowl2021adversarial} add a label-related imperceptible noise to distract the model from extracting the feature of original images. This kind of noise has an obvious connection with the ground truth label and works as a shortcut. Deep neural networks prefer to extract such easy-to-learn shortcut features and ignore more complicated semantic information in the original images\cite{geirhos2020shortcut}. Shan et al.~\cite{shan2020fawkes} applied this method to a more specific domain, fact recognition. He et al.~\cite{he2022indiscriminate} change this method from a supervised manner into the unsupervised manner to protect an unlabeled dataset from unauthorized using by contrasive learning~\cite{chen2020simple, grill2020bootstrap, chen2020improved}. 

However, all the unlearnable methods above can only work under one single training setting. More specifically, the unlearnable examples generated in a supervised way can protect data from supervised training, but cannot work when others train with it in an unsupervised way and vice versa. This exposes the data almost unprotected since we are not able to control how the attackers who collected our data will use it. As shown in Figure~\ref{intro_pic}, the error-minimizing noise (EMN)~\cite{huang2020unlearnable} is only used for supervised learning and can not work under unsupervised learning, while Unsupervised Contrastvive Learning (UCL) is only used for unsupervised learning and can not work in the other learning. This problem shows the importance to protect data in a more comprehensive way. For protecting the data from being used without permission by both supervised learning and unsupervised learning, we proposed a general unlearnable noise in this paper, which can stop the models from learning the image features in both training manners.

\begin{figure}
  \label{intro_pic}
  \centering
  \includegraphics[width=250pt]{pic/intro4.png}
  \caption{Accuracy on clean test data of different unlearnable examples trained by supervised model and unsupervised model}
\end{figure}

We first find that the unlearnable perturbation generated in supervised way~\cite{huang2020unlearnable} can not work under unsupervised learning like SimCLR~\cite{chen2020simple}. If the unauthorized third party uses unsupervised learning to pre-train on the unlearnable dataset, it can break the unlearnable perturbation. Also, the perturbation generated in unsupervised way~\cite{he2022indiscriminate} will lose the unlearnable effect under the supervised training. So for protect the data from unauthorized using in a more comprehensive way, inspired by~\cite{yu2021indiscriminate} which shows that linear separable features can be a shortcut for supervised unlearnable examples, we proposed a method to add the property of linear separability to the perturbation generated in unsupervised way. In this way, we are able to make a labeled dataset unlearnable in both supervised learning and unsupervised learning. 

Besides the general unlearnable examples on annotated datasets, we further propose the method of using $k$-kmeans pseudo labels to extend unlearnable examples to unlabeled data, which decreases the accuracy in supervised training by \textcolor{red}{10\%} and boosted the unlearnable contrastive learning to a higher level, in case other people collect and annotate it to train their model without permission. We also found the special trade-off between the between supervised and self-supervise components in the perturbation. It is not just competing with each other. When we put more weight on one of the components, the other light component will have positive influence on the weight one instead of decreasing its performance.

Our contributions are summarized as follows:
\begin{itemize}
    \item We proposed a general unlearnable method that can extend unlearnable examples of the labeled dataset to both the supervised learning and the self-supervised learning, which can prevent the data from unauthorized using comprehensively in both cases.
    \item We generalize this idea to the unlabeled datasets by pseudo label. When label information is not available, we can use $k$-means to get the pseudo label. Although we can decrease the performance by just 10\% in supervised learning, the performance of unlearnable contrastive learning can be enhanced. 
    % \item We have noticed that the trade-off between supervised and self-supervised unlearnable components n is not just competing with each other. When we put more weight on one of the components, the other light component will have positive influence on the weight one. %(It is possible that transferbility from resnet-18 to VGG11 is also better than supervised unlearnable baseline. I am doing experiments to verify.)
\end{itemize}

% 52734685 53113236


==> sections/unused_HAN.tex <==
\textbf{Training-wise Transferability.} Previous methods protect data from one single training setting, either supervised training~\cite{huang2020unlearnable} or unsupervised training~\cite{he2022indiscriminate}. In supervised training, the unlearnable examples are designed to make the classifier, $f_\theta$, trained on it to have a low accuracy on clean test data. In unsupervised training, the unlearnability is to produce a poor feature extractor, $g_\eta$, such that any data fine-tuned on it cannot perform well on clean test data. The transferability between different training settings means that both $f_\theta$ trained in a supervised way and $g_\eta$ trained in an unsupervised way have a low classification accuracy on test dataset.

\textbf{Data-wise Transferability.}
Under the setting of supervised training, when any other dataset, $\cD_{\tilde{c}} = \{(\tilde{\vx}_i, \tilde{y}_i)\}_{i=1}^{\tilde{n}}$, where $\tilde{\vx}_i \in \tilde{\mathcal{X}} \subset \RR^d$ and $\tilde{y}_i \in \tilde{\mathcal{Y}} = \{1, 2, \dots, \tilde{K}\}$, also requires protection, it would be efficient if we can transfer the perturbation that is already generated for $\cD_{c}$ onto $\cD_{\tilde{c}}$. If the perturbation, $\Delta_{\cD_c}$, is data-wise transferable, the unlearnable training dataset, $\cD_{\tilde{u}}$, for $\cD_{\tilde{c}}$ can be constructed as 
\begin{align}
\label{eq:datawise_transfer}
    \cD_{\tilde{u}}=\{(\tilde{\vx}_i + \vdelta_{H(i)}, \tilde{y}_i)\}_{i=1}^n,
\end{align}
where $~\tilde{\vx}_i\in \cD_{\tilde{c}}$, $\vdelta_{H(i)} \in \Delta_{\cD_c}$, and $H(i)$ decides which perturbation in $\Delta_{\cD_c}$ is added on $~\tilde{\vx}_i$ in the new dataset, $\cD_{\tilde{c}}$. If the perturbations are data-wise transferable, the classifier, $f_{\tilde{\theta}}$, trained on $\cD_{\tilde{u}}$ also performs poorly on test data. % It is possible that $\cD_{\tilde{c}}$ has more classes than $\cD_c$, i.e. $\tilde{K} > K$, or the number of samples is larger than 


\begin{table}[h]
  \caption{Unlearnable Examples Settings of Existing Approaches}
  \label{tab:setting}
  \centering
%   \begin{threeparttable}
  \begin{tabular}{cc|cc}
    \toprule
    Dataset Setting & Protected by & Supervised Training & Unsupervised Training \\
    \midrule
    \multirow{2}*{Labeled} & Supervised Unlearnability & \cite{huang2020unlearnable,fowl2021adversarial} & \xmark  \\
    \cmidrule{2-4}
    & Unsupervised Unlearnability & \xmark & \cite{he2022indiscriminate} \\
    \midrule
    % Unsupervised Setting & \xmark & \cmark \\
    % \multirow{2}*{Unlabeled} & Supervised Unlearnability & \xmark & \xmark \\
    Unlabeled & Unsupervised Unlearnability & \xmark & \cite{he2022indiscriminate} \\
    \bottomrule
  \end{tabular}
%   \end{threeparttable}
\end{table}



\subsection{Linear Separability and Transferability}
\label{sec:pre_linear_sep}

% \jt{Linear Separability is important for transferability but existing ones are not sufficient? }

It is claimed by Yu et al.~\cite{yu2021indiscriminate} that in supervised learning, if the perturbation is linear separable between different classes, it can lead to unlearnable examples. They think this linear separability is the easy-to-learn feature of unlearnable examples, but we found that linear separability is not the only reason behind previous unlearnable methods. We also found that Synthetic Noise, which is manually designed based on linear separability, is data-wise transferable. This shows that it is possible to use linear separability to realize data-wise transferability. However, SN cannot be embedded in other optimization objective for transferring on different training settings. So we want to propose an optimizable linear separability objective that allows make the unlearnable examples data-wise and training-wise transferable.

\subsubsection{Linear Separability vs. Unlearnability}
\label{sec:pre_linear_vs_unlearn}
According to Yu et al.~\cite{yu2021indiscriminate}, in supervised learning, unlearnable examples create linear separability, that the label-related imperceptible perturbation is linearly separable between different classes, as a shortcut for the optimization objective. They got this conclusion from the observation that, in the input space, the perturbations for the same class are well clustered, which causes that the imperceptible perturbation is much easier to be classified even by a linear model than the semantic features in clean samples. Note that the linear separability is only about $\vdelta_i$ and $y_i$, and not related to $\vx_i$. Thus, the neural networks tend to extract the perturbations as the dominant features. However, from the preliminary experiment in Table~\ref{tab:cifar100_correspond}, we found that linear separability can produce unlearnable examples, but is not equivalent to unlearnability. 

Table~\ref{tab:cifar100_correspond} shows that even though the linear separability and $\mathcal{D}_{c}$ are the same, the unlearnable effect can be very different.
By setting $y_{s_{\text{inter}}(i)} = y_{s_{\text{inter}}(j)}$ if $y_i = y_j$, and $y_{s_{\text{inter}}(i)} \neq y_{s_{\text{inter}}(j)}$ if $y_i \neq y_j$, we first keep the linear separability unchanged after $s_{\text{inter}}(i)$, the inter-class corresponding swapping. This operation results in if two perturbations correspond to the examples from the same class, they are assigned to two examples from another class after being changed by $s_{\text{inter}}(i)$. It means that we swap the perturbations of the whole class to another class. So the clustering and linear separability is not changed after $s_{\text{inter}}(i)$, while for $s_{\text{intra}}(i)$, it is naturally unchanged.
In this way, we keep examples and the linear separability of perturbations the same as those before swapping. As shown in Table~\ref{tab:cifar100_correspond}, although the linear separability is not changed, the unlearnable effect becomes weak. The perturbation generated by EMN works best when it is added on the target example. It implies that the linear separability is not the only reason behind unlearnable examples that are based on the optimization like EMN.

To our supervise, Synthetic Noise~\cite{yu2021indiscriminate} in Table~\ref{tab:cifar100_correspond}, a manually designed linear separable perturbation, is not affected by $s_{\text{inter}}(i)$ and $s_{\text{intra}}(i)$. It is generated by linear separability and is independent on target data, so SN is not weakened when added on non-target data.
% In fact, we find that linear separability can lead to unlearnability that is data-wise transferable but also has its own weaknesses. 
In fact, although linear separability is not the only factor of optimization-based methods like EMN, the perturbation that is totally based on linear separability can lead to unlearnable effect. And this unlearnability is data-wise transferable. But Synthetic Noise also has its own weakness.
In Section~\ref{sec:SN_problem}, we discussed the weakness of Synthetic Noise. Then in Section~\ref{sec:sepa_loss}, we propose the new Clustering Separability Discriminant to make use of the data-wise transferability of the linear separability and overcome its weakness.

\begin{table}[h]
  \caption{Test accuracy (\%) on CIFAR100 with different correponding between train data and perturbations.}
  \label{tab:cifar100_correspond}
  \centering
%   \begin{threeparttable}
  \begin{tabular}{ccc}
    \toprule
    Corresponding & EMN~\cite{huang2020unlearnable} & Synthetic Noise~\cite{yu2021indiscriminate} \\
    \midrule
    original & 6.59 & 2.13 \\
    $s_{\text{intra}}$ & 21.63 & 2.44 \\
    $s_{\text{inter}}$ & 35.50 & 2.73 \\
    \bottomrule
  \end{tabular}
%   \end{threeparttable}
\end{table}

\subsubsection{The Shortcoming of linear separable Synthetic Noise}
\label{sec:SN_problem}

Although Synthetic Noise (SN)~\cite{yu2021indiscriminate} can lead to data-wise transferability, it has its own shortcoming. Synthetic Noise is generated by sampling from a manually designed distribution. This distribution is totally based on the artificial design and has no quantitative metrics. 
We cannot embed the linear separability into other methods like UCL, since the sampling process is incompatible with an optimization process. But to induce the unlearnable examples to have data-wise and training-wise transferability at the same time, the linear separability should be quantified for being embedded into other optimization process. So in the following sections, we propose an quantifiable linear separability to generate it from an optimizable process instead of sampling. With the optimizable linear separability, we can make the unlearnability transferable on different datasets and, meanwhile, embedding linear separability into unsupervised unlearnable examples to make it transferable under different training settings.

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.8\textwidth]{pic/SN_acc.png}
%   \caption{Accuracy on CIFAR100 test data and loss during the training on unlearnable training data.}
%   \label{fig:SN_acc}
% \end{figure}


\begin{figure}[t]
  \centering
  \includegraphics[width=0.55\textwidth]{pic/emn_sn_tsne2.png}
  \caption{t-SNE visualization of EMN and SN in input space}
  \label{emn_sn_tsne}
\end{figure}
